QCSHQD: Quantum computing as a service for Hybrid classical-quantum software development: A Vision

Quantum Computing (QC) is transitioning from theoretical frameworks to an indispensable powerhouse of computational capability, resulting in extensive adoption across both industrial and academic domains. QC presents exceptional advantages, including unparalleled processing speed and the potential to solve complex problems beyond the capabilities of classical computers. Nevertheless, academic researchers and industry practitioners encounter various challenges in harnessing the benefits of this technology. The limited accessibility of QC resources for classical developers, and a general lack of domain knowledge and expertise, represent insurmountable barrier, hence to address these challenges, we introduce a framework- Quantum Computing as a Service for Hybrid Classical-Quantum Software Development (QCSHQD), which leverages service-oriented strategies. Our framework comprises three principal components: an Integrated Development Environment (IDE) for user interaction, an abstraction layer dedicated to orchestrating quantum services, and a service provider responsible for executing services on quantum computer. This study presents a blueprint for QCSHQD, designed to democratize access to QC resources for classical developers who want to seamless harness QC power. The vision of QCSHQD paves the way for groundbreaking innovations by addressing key challenges of hybridization between classical and quantum computers.

==> Sections/Implementation_consideration_and_discussion.tex <==
This section details the tools and methodologies for implementing QCSHQD. We plan to extend the PyDev plugin\footnote{\url{https://www.pydev.org/}} for Eclipse to develop the IDE. Furthermore, for version control and research data management, the project will integrate Git \footnote{\url{https://git-scm.com/}}, which can be effectively used within the Eclipse environment through existing Git plugins.

The abstraction layer design is based on the work of \citet{valencia2021hybrid} and \citet{weder2021hybrid} through OpenAPI\footnote{\url{https://www.openapis.org/}} and TOSCA-based orchestration \cite{lipton2017oasis}. The role of a TOSCA-based orchestration mechanism, \cite{weder2021hybrid,lipton2017oasis} will be automating the process of translating classical input to quantum-compatible formats, selecting appropriate quantum computers, handling the deployment of quantum computing services, interpreting the quantum data and translating them back into classical representation of the results.
The OpenAPI offers a standardized specification for developing and generating APIs to ensure seamless task execution and data integrity. The importance of OpenAPI not only can be defined in users' understanding and exploring services' capabilities, but it will also facilitate services development. Its specification needs to be modified to support quantum services \cite{romero2023enabling}, therefore, we plan to utilize OpenAPI with an extension, considering custom properties tailored specifically for defining quantum applications. These custom properties serve as a means to incorporate supplementary information into the API contract definition, expanding the scope of the specification \cite{romero2023enabling}.

Our primary deployment targets are QC services available on the cloud as well as real-world QC infrastructure, such as VTT quantum computer HELMI connected with CSC LUMI\footnote{\url{https://www.csc.fi/lumi}} for QC provider, which depends on the evolving situation of QC.

Future efforts will be put into defining and evaluating the existing process for developing quantum software based on the QCSHQD. To anticipate this task, we benefit from continuous software engineering practices for team collaboration, short development iterations, and continuous delivery \cite{fitzgerald2017continuous}.



\subsection{Potential Limitations }

QC is still a new domain, and technologies are quickly evolving. Therefore, in this work, we foresee a set of possible scenarios that might impact the proposed road-map. 

\begin{itemize}
    \item The \textbf{integration} of quantum computing services with classical systems may encounter compatibility issues due to the quantum infrastructure readiness.
\item \textbf{Allocation of quantum resources} in a cloud-based service model could be complex, in case of high demand for quantum computing power.

\item \textbf{Scalability: }As the demand for quantum computing resources grows, the framework might face scalability issues.
\item \textbf{Evolution of Quantum Technologies:} The rapidly evolving nature of quantum computing technologies may outpace the development of the proposed framework, necessitating continuous updates and adaptations.


\end{itemize}
